The influence of van der Waals interactions on a bubble moving in a tube

We consider the unsteady thin-film dynamics of a long bubble of negligible viscosity that advances at a uniform speed in a cylindrical capillary tube. The bubble displaces a viscous, nonwetting fluid, creating a thin film between its interface and the tube walls. The film is considered thin enough that intermolecular forces in the form of van der Waals attractions are significant and thin-film rupture is possible. In the case of negligible intermolecular forces, a steady-state solution exits where a film of uniform thickness is deposited in the annular region between the bubble interface and the tube walls. However, once intermolecular interactions are important, the interface is perturbed out of its steady state and either (i) the perturbation grows sufficiently before reaching the rear meniscus of the bubble such that rupture occurs; or (ii) the perturbation remains small due to weak intermolecular forces until it leaves the bubble interface through the rear meniscus. We obtain, both numerically and asymptotically, the time-scale over which rupture occurs, and thus, we find a critical capillary number, depending on the bubble length and the strength of the intermolecular forces, below which the film is predicted to rupture.

==> caption/CHANGELOG <==
caption package
===============

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added


bicaption package
=================

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added


ltcaption package
=================

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
==================

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption


newfloat package
================

v1.0 (2011/10/30)
- 1st published version

v1.1 (2013/04/27)
- New command \PrepareListOf


totalcount package
==================

v1.0 (2008/03/09)
- 1st published version



==> caption/README <==
==========================================================================

The `caption' package bundle
Release 2016-05-22
Copyright (C) 1994-2016 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  http://sourceforge.net/projects/latex-caption/

If you need help for installation please visit:
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=inst-miktex*
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=installthings
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=privinst

If you need help using these packages please visit:
  http://www.latex-community.org/
  http://tex.stackexchange.com/
  http://www.golatex.de/           (German)
  http://www.texwelt.de/           (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  http://sourceforge.net/p/latex-caption/tickets/
or send an e-mail to me
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.3 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.1 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.1 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

The `newfloat' package v1.1 offers the command \DeclareFloatingEnvironment
for defining new floating environments which behave like the existing
floating environments "figure" and "table".

User Manual: newfloat.pdf (English)

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)

